Translating HOL to Dedukti

Dedukti is a logical framework based on the lambda-Pi-calculus modulo rewriting, which extends the lambda-Pi-calculus with rewrite rules. In this paper, we show how to translate the proofs of a family of HOL proof assistants to Dedukti. The translation preserves binding, typing, and reduction. We implemented this translation in an automated tool and used it to successfully translate the OpenTheory standard library.

==> eptcsdata.tex <==
\providecommand{\firstpage}{74}
\providecommand{\publicationstatus}{C.Kaliszyk and A. Paskevich (Eds.): 4th Workshop\\
on Proof eXchange for Theorem Proving (PxTP'15).\\
EPTCS 186, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.186.8}{10.4204/EPTCS.186.8}}
\pdfoutput=1

